Nonparametric Identification and Estimation with Non-Classical Errors-in-Variables

This paper considers nonparametric identification and estimation of the regression function when a covariate is mismeasured. The measurement error need not be classical. Employing the small measurement error approximation, we establish nonparametric identification under weak and easy-to-interpret conditions on the instrumental variable. The paper also provides nonparametric estimators of the regression function and derives their rates of convergence.

==> named_thm_preamble.tex <==

\makeatletter
\def\namedlabel#1#2{\begingroup
   \def\@currentlabel{#2}   \label{#1}\endgroup
}

\RequirePackage{ifthen}
\newtheoremstyle{namedAssumption}{}{}{\itshape}{}{\bfseries}{.}{.5em}{#1 \ifthenelse{\equal{#3}{}}{{#2}}{{#3}}} 
\makeatother

